(Un)Decidability Results for Word Equations with Length and Regular Expression Constraints

We prove several decidability and undecidability results for the satisfiability and validity problems for languages that can express solutions to word equations with length constraints. The atomic formulas over this language are equality over string terms (word equations), linear inequality over the length function (length constraints), and membership in regular sets. These questions are important in logic, program analysis, and formal verification. Variants of these questions have been studied for many decades by mathematicians. More recently, practical satisfiability procedures (aka SMT solvers) for these formulas have become increasingly important in the context of security analysis for string-manipulating programs such as web applications. We prove three main theorems. First, we give a new proof of undecidability for the validity problem for the set of sentences written as a forall-exists quantifier alternation applied to positive word equations. A corollary of this undecidability result is that this set is undecidable even with sentences with at most two occurrences of a string variable. Second, we consider Boolean combinations of quantifier-free formulas constructed out of word equations and length constraints. We show that if word equations can be converted to a solved form, a form relevant in practice, then the satisfiability problem for Boolean combinations of word equations and length constraints is decidable. Third, we show that the satisfiability problem for quantifier-free formulas over word equations in regular solved form, length constraints, and the membership predicate over regular expressions is also decidable.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
Algorithms for deciding the satisfiability problem for formulas about
strings are crucial for many software reliability and security
applications. However, many theoretical questions regarding theories
of strings remain open. In this paper we prove two results. First, we
show that the satisfiability problem for $B\Lelr{0}$ formulas is
undecidable. Second, the satisifiability problem for $\Lel{0}$
formulas is decidable, provided that there is an algorithm to obtain
the solved forms of given word equations.


==> evaluation.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.1}
\centering
%\textsf{
\begin{tabular}{|l|l|p{0.8cm}|p{0.8cm}|p{1.5cm}|p{1.5cm}|p{1.4cm}|}
  \hline
  &\bf{ Num. of Roles, Rules} & \multicolumn{1}{c|}{\bf{MC}} &
   \multicolumn{1}{c|}{\bf{BMC}}  &  \multicolumn{2}{c|}{\bf{RBAC-PAT}} 
  & \multicolumn{1}{c|}{\bf{\mohawk}} \\
\cline{5-6}
  &  & & & {Forward reachability} & {Backward reachability}
  & \\
  \hline
  1. & 3, 15 & \rgt{0.097s} & \rgt{0.016s} & \rgt{0.625s}  & \rgt{0.240s} & \rgt{0.382s} \\
  2. & 5, 25 & \rgt{0.050s} & \rgt{0.025s} & \rgt{0.695s}  & \rgt{0.281s} & \rgt{0.431s} \\
  3. & 20, 100 & \rgt{M/O} & \rgt{0.103s} & \rgt{0.806s}  & \rgt{Err} & \rgt{0.733s}\\ 
  4. & 40, 200 &  \rgt{M/O}  & \rgt{0.110s} & \rgt{0.780s} & \rgt{Err} & \rgt{0.379s} \\
  5. & 200, 1000 & \rgt{M/O} & \rgt{0.624s} & \rgt{1.471s} & \rgt{Err} & \rgt{0.477s} \\
  6. & 500, 2500 & \rgt{M/O} & \rgt{3.2s} & \rgt{2.177s} & \rgt{Err}
  & \rgt{0.531s} \\
  7. & 4000, 20000 & \rgt{M/O} & \rgt{414s} & \rgt{7.658s} &
  \rgt{Err} & \rgt{3.138s} \\
  8. & 20000, 80000 & \rgt{M/O} & \rgt{M/O} & \rgt{110s}
  & \rgt{Err} & \rgt{53s} \\
% 9. & 30000, 120000 & \rgt{M/O} & \rgt{M/O} & \rgt{210s}
%  & \rgt{Err} & \rgt{134s} \\
%  10. & 100000, 40000, 200000 & \rgt{M/O} & \rgt{M/O} & \rgt{6m 16s} & \rgt{M/O}
%  & \rgt{4m 32s} \\
%  11. & 150000, 80000, 400000 & \rgt{T/O} & \rgt{T/O} & \rgt{22m 58s}
%  & \rgt{M/O}& \rgt{42m 34s} \\  
  \hline
\end{tabular}
\centering
\scriptsize{
\begin{tabular}{lcllcllcl}
%\multicolumn{6}{c}{\textbf{Legend}}\\
  m &-& minutes & MC & - & NuSMV symbolic model checking & T/O & - &
  Time out after 60 mins \\
 s & - & seconds & BMC & - & NuSMV bounded model checking & M/O & - &
 Memory out \\
 ms & - & milliseconds & RBAC-PAT & - & Tool from Stoller et
  al.~\cite{scott07,rbacpat} & Err & - & Segmentation fault\\
  \end{tabular}
}
\caption{Evaluation of error-finding tools on positive conjunctive
  ARBAC policies. (Test suite 1) \label{tab:pos}}
%}
\end{table*}


\begin{table*}[ht]
\renewcommand{\arraystretch}{1.1}
\centering
\footnotesize{
\begin{tabular}{|l|l|p{0.8cm}|p{0.8cm}|p{1.5cm}|p{1.5cm}|p{1.4cm}|}
  \hline
  &\bf{ Number of Roles, Rules} & \multicolumn{1}{c|}{\bf{MC}} &
   \multicolumn{1}{c|}{\bf{BMC}}  &  \multicolumn{2}{c|}{\bf{RBAC-PAT}} 
  & \multicolumn{1}{c|}{\bf{\mohawk}} \\
\cline{5-6}
  &  & & & {Forward reachability} & {Backward reachability}
  & \\
  \hline
  1. & 3, 15 & \rgt{0.022s} & \rgt{0.021s} & \rgt{0.513s}  & \rgt{0.241s} & \rgt{0.442s} \\
  2. & 5, 25  & \rgt{0.064s} & \rgt{0.026s}  & \rgt{0.519s} & \rgt{0.252s} & \rgt{0.501s} \\
  3. & 20, 100 & \rgt{M/O} & \rgt{0.048s} & \rgt{0.512s} & \rgt{Err} & \rgt{0.436s} \\
  4. & 40, 200 & \rgt{M/O} & \rgt{0.122s} & \rgt{0.534s} & \rgt{Err} & \rgt{1.303s} \\
  5. & 200, 1000 & \rgt{M/O} & \rgt{0.472s} & \rgt{0.699s} & \rgt{Err} & \rgt{0.504s} \\
  6. & 500, 2500 & \rgt{M/O} & \rgt{1.819s} & \rgt{2.414s} &
  \rgt{Err}& \rgt{0.597s} \\
  7. & 4000, 20000 & \rgt{M/O} &
  \rgt{109s} & \rgt{311s} & \rgt{Err} & \rgt{2.753s} \\
  8. & 20000, 80000 & \rgt{M/O} &
  \rgt{M/O} & \rgt{T/O} &  \rgt{Err} & \rgt{40s} \\
%  9. & 30000, 130000 & \rgt{M/O} & \rgt{M/O} & \rgt{T/O} &
%  \rgt{Err} & \rgt{99s} \\
%  10. & 100000, 40000, 200000 & \rgt{M/O} &
%  \rgt{M/O} & \rgt{T/O}  & \rgt{Err} & \rgt{ 252s} \\
%  11. & 150000, 80000, 400000 & \rgt{T/O} & \rgt{T/O} & \rgt{T/O}   &
%  \rgt{M/O} & \rgt{41m 23s} \\  
\hline
\end{tabular}
}
\scriptsize{
\begin{tabular}{lcllcllcl}
%\multicolumn{6}{c}{\textbf{Legend}}\\
  m &-& minutes & MC & - & NuSMV symbolic model checking & T/O & - &
  Time out after 60 mins \\
 s & - & seconds & BMC & - & NuSMV bounded model checking & M/O & - &
 Memory out \\
 ms & - & milliseconds & RBAC-PAT & - & Tool from Stoller et
  al.~\cite{scott07,rbacpat} & Err & - & Segmentation fault\\
\end{tabular}
}
\caption{Evaluation of error-finding tools on mixed conjunctive ARBAC
  policies with no \canRevoke rules. (Test suite 2) \label{tab:mixednocr}}
\end{table*}

\begin{table*}[ht]
\renewcommand{\arraystretch}{1.1}
\centering
\footnotesize{
\begin{tabular}{|l|l|p{0.8cm}|p{1cm}|p{1.5cm}|p{1.5cm}|p{1.4cm}|}
  \hline
  &\bf{Num. of Roles, Rules} & \multicolumn{1}{c|}{\bf{MC}} &
   \multicolumn{1}{c|}{\bf{BMC}}  &  \multicolumn{2}{c|}{\bf{RBAC-PAT}} 
  & \multicolumn{1}{c|}{\bf{\mohawk}} \\
\cline{5-6}
  &  & & & {Forward reachability} & {Backward reachability}
  & \\
  \hline
  1. & 3, 15 & \rgt{0.030s} & \rgt{0.102s} & \rgt{1.452s}  & \rgt{0.665s} & \rgt{0.380s} \\
  2. & 5, 25  & \rgt{0.044s} & \rgt{0.033s}  & \rgt{1.666s} & \rgt{0.881s} & \rgt{0.431s} \\
  3. & 20, 100 & \rgt{M/O} & \rgt{0.056s} & \rgt{1.364s} & \rgt{Err} & \rgt{0.381s} \\
  4. & 40, 200 & \rgt{M/O} & \rgt{0.169s} & \rgt{1.476s} & \rgt{Err} & \rgt{0.984s} \\
  5. & 200, 1000 & \rgt{M/O} & \rgt{0.972s} & \rgt{2.258s} & \rgt{Err} & \rgt{0.486s} \\
  6. & 500, 2500 & \rgt{M/O} & \rgt{2.422s} & \rgt{7.350s} &
  \rgt{Err}& \rgt{0.487s} \\
  7. & 4000, 20000 & \rgt{M/O} &
  \rgt{109s} & \rgt{511s} & \rgt{Err} & \rgt{2.478s} \\
  8. & 20000, 80000 & \rgt{M/O} &
  \rgt{M/O} & \rgt{T/O} &  \rgt{Err} & \rgt{41s} \\
% 9. & 30000, 130000 & \rgt{M/O} & \rgt{M/O} & \rgt{T/O} &
%  \rgt{Err} & \rgt{99s} \\
%  10. & 100000, 40000, 200000 & \rgt{T/O} &
%  \rgt{T/O} & \rgt{T/O}  & \rgt{M/O} & \rgt{ 3m 35s} \\
%  11. & 150000, 80000, 400000 & \rgt{T/O} & \rgt{T/O} & \rgt{T/O}   &
%  \rgt{M/O} & \rgt{32m 5s} \\  
\hline
\end{tabular}
}
\scriptsize{
\begin{tabular}{lcllcllcl}
%\multicolumn{6}{c}{\textbf{Legend}}\\
  m &-& minutes & MC & - & NuSMV symbolic model checking & T/O & - &
  Time out after 60 mins \\
 s & - & seconds & BMC & - & NuSMV bounded model checking & M/O & - &
 Memory out \\
 ms & - & milliseconds & RBAC-PAT & - & Tool from Stoller et
  al.~\cite{scott07,rbacpat} & Err & - & Segmentation fault\\
\end{tabular}
}
\caption{Evaluation of error-finding tools on mixed conjunctive ARBAC
  policies. (Test suite 3) \label{tab:mixed}}
\end{table*}

\begin{table*}[!ht]
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{|l|l|p{0.8cm}|p{0.8cm}|p{1.5cm}|p{1.5cm}|p{1.4cm}|}
  \hline
  & \bf{ Num. of Roles, Rules} & \multicolumn{1}{c|}{\bf{MC}} &
  \multicolumn{1}{c|}{\bf{BMC}}  &  \multicolumn{2}{c|}{\bf{RBAC-PAT}} 
  &  \multicolumn{1}{c|}{\bf{\mohawk}}  \\
 % \cline{3-8}
\cline{5-6}
  & & & & {Forward reachability}
  & {Backward reachability}
  & \\
  \hline
  1. & 12, 19 & \multicolumn{1}{r|}{0.025s} & \rgt{0.022s} & \rgt{0.531s} & \rgt{0.238s} & \rgt{0.300s}\\
  2. & 20, 266 & \rgt{0.023s} & \rgt{0.026s} &
  \rgt{0.559s} & \rgt{0.247s} & \rgt{0.400s} \\
  3. & 32, 162 & \rgt{M/O} & \rgt{0.182s} & \rgt{1.556s} & \rgt{0.568s} &
  \rgt{0.830s} \\
  \hline
\end{tabular}
\scriptsize{
\begin{tabular}{lcllcllcl}
%\multicolumn{6}{c}{\textbf{Legend}}\\
  m &-& minutes & MC & - & NuSMV symbolic model checking & T/O & - &
  Time out after 60 mins \\
 s & - & seconds & BMC & - & NuSMV bounded model checking & M/O & - &
 Memory out \\
 ms & - & milliseconds & RBAC-PAT & - & Tool from Stoller et
  al.~\cite{scott07,rbacpat} & Err & - & Segmentation fault\\
  \end{tabular}
}
\caption{ Evaluation of error-finding tools on ARBAC policies obtained from
  previous literature.}
\label{tab:simple}
\end{table*}


\section{Results}
\label{sec:evaluation}

The objective of our experiments was to ascertain the effectiveness of
the abstraction-refinement technique implemented in \mohawk, and
compare it with existing state-of-the-art methods for finding errors
in access-control policy, namely symbolic model checking, bounded
model checking, and RBAC-PAT~\cite{scott07}. We chose
NuSMV~\cite{nusmv} as the reference implementation for both symbolic
and bounded model checking. Note that although all the competing
techniques were developed in the verification context, they can also
be used for the purposes of error finding. In the following, we will
use the terms MC and BMC to refer to NuSMV's symbolic model checker
and NuSMV's bounded model checker respectively. All the experiments
were conducted on Macbook Pro laptop with Intel Core 2 Duo 2.4GHz
processor and 4GB RAM.

\subsection{Benchmarks Used}

We have used two sets of policies to evaluate the various tools.  Both
are based on prior
work~\cite{schaad01,molloy09,jha07,scott07,rbacpat}.  The first set
has not been used previously; we built it based on data from RBAC
deployments~\cite{schaad01}, and benchmarks used in role
mining~\cite{molloy09}. The second has been used in the context of
verification of ARBAC policies in prior work~\cite{scott07,rbacpat}
(These policies are simpler compared to the policies in the first
set).

\textbf{Complex Policies (Set 1):} We built three test suites of
policies that were designed to factor in the known sources of
complexity, be reflective of the sizes of policies we expect to see in
real deployments, and exercise the full expressiveness of ARBAC. As
explained in section \ref{sec:complexity} and
Appendix~\ref{app:sources:complexity}, the four known sources of
complexity in ARBAC policies are disjunctions in the \canAssign rules,
number of positive preconditions, number of mixed preconditions, and
number of irrevocable roles. Jha et al.~\cite{jha07} provides the
restrictions under which safety analysis for ARBAC, which is the
error-finding problem in our context, is PSPACE-Complete, NP-Complete,
and solvable in polynomial time. Accordingly, we created three test
suites:
\begin{itemize}
\item {\bf Test suite 1:} Policies with positive conjunctive
  \canAssign rules and non-empty \canRevoke rules. Error-finding
  problem is solvable in polynomial time for these policies.

\item {\bf Test suite 2:} Policies with mixed conjunctive \canAssign
  rules and empty \canRevoke rules. Error-finding problem is
  NP-Complete for these policies.

\item {\bf Test suite 3:} Policies with mixed conjunctive \canAssign
  rules and non-empty \canRevoke rules. Error-finding problem is
  PSPACE-Complete for these policies.
\end{itemize}

The preconditions for the \canAssign rules were randomly
created. Unlike the policies in Set 2 obtained
from~\cite{scott07,rbacpat}, these policies may have more than one
positive precondition per \canAssign rule.

We implemented a policy-generation tool that accepts the following
inputs, namely number of users, number of roles, number of \canAssign
rules, number of \canRevoke rules, type of can\_assign rules, and type
of UA, and dumps an ARBAC policy into an output file. The generated
policies have an administrative role and an administrative user
assigned to administrative role, by default. The administrative role
is used in all the \canAssign rules. The \canRevoke rules can be
chosen to be either positive conjunctive or mixed. The initial UA can
be either empty or randomly assigned. For each policy, the
reachability of a role by a user is random. Also, for each policy, the
tool creates a safety question at random. The safety question asks
whether a role is reachable by a user.

In these policies we are hoping to capture the typical security intent
of a system administrator, namely, a subset of users may not reach a
subset of roles. Since the policies are randomly built, it is possible
that some randomly generated rules allow for a user to eventually
reach a designated role, i.e., the policy may have an error. It is
these kind of policies that interest us. 

% Since the policies are
% randomly generated, it is possible that no user may reach the
% designated role. In such an event, we do not consider these policies
% for experimental evaluation since we are interested only in policies
% with errors in them. It is also possible that the user we chose for
% the safety question cannot reach the designated role. If so, we
% randomly generate a new safety question.

\textbf{Simple Policies (Set 2):} We used three ARBAC policies used in
previous work for the evaluation of the verification tool,
RBAC-PAT~\cite{scott07,sasturkar06,rbacpat}. The first policy is an
ARBAC policy for a hypothetical hospital, while the second policy is
for a hypothetical university. The third policy from~\cite{rbacpat} is
a test case having mixed preconditions. The first two policies were
used in~\cite{scott07} for case studies. The third policy was used in
~\cite{rbacpat}, and a complete state-space exploration took 8.6 hours
in RBAC-PAT.  An important restriction in these policies is that they
have atmost one positive pre-condition per \canAssign rule. As we will
explain later, answering the safety question for these policies was
fairly easy for all the tools.

\subsection{Experimental Methodology}
In all the experiments, the input to the error-finding tools consisted
of an ARBAC policy and a safety question. We applied the static
slicing techniques on all the policies prior to the experiments. The
policies were encoded using the input language of the respective
tools. MC and BMC use the SMV finite state machine language, while
RBAC-PAT and \mohawk have their own input language. We implemented a
translation tool to convert policies in \mohawk's input language to
both SMV and RBAC-PAT input languages. We expected the tools to
conclude that the role is reachable and provide the sequence of
administrative actions that lead to the role assignment. In our
evaluation, we had two users for each policy, namely the user in the
safety question and the administrator. These are the only users
required for answering the safety question. Moreover, static slicing
techniques also remove the users who are not connected to the safety
question.

\subsection{Results Explained}

We explain the results of our experimental evaluation below. Whenever
we refer to \mohawk below, we mean \mohawk configured with aggressive
abstraction-refinement, unless specified otherwise.

\subsubsection{\bf Results on Complex Policies}

The results of our evaluation on complex policies (Set 1) are
tabulated in Table~\ref{tab:pos} (Test suite 1),
Table~\ref{tab:mixednocr} (Test suite 2), and Table~\ref{tab:mixed}
(Test suite 3). Static slicing was not effective for the policies in
our test suite. This is because the randomly built preconditions for
the \canAssign rules may relate a majority of the roles in the
policies to one another. 

Our results indicate that \mohawk scales better than all the competing
tools, irrespective of the complexity of the input policy. BMC scales
better than MC, but still runs out of memory for policy \#8 in all the
test suites. RBAC-PAT's forward reachability, although slower compared
to BMC, is effective for test suite 1, whose policies are verifiable
in polynomial time. However, RBAC-PAT's forward reachability times out
for policy \#8 in test suites 2 and 3. The forward reachability
algorithm in RBAC-PAT can be considered as a specialized model
checking algorithm for ARBAC policies, and scales better than symbolic
model checking. RBAC-PAT's backward reachability algorithm was faster
compared RBAC-PAT's forward algorithm for policies 1 and 2 in all the
test suites, but gave a segmentation fault for all policies 3-8 in all
the test suites. It is unclear whether this is because of a bug in the
implementation or if the tool ran out of memory. \mohawk scales better
compared to all the tools, and is orders of magnitude faster than
competing tools for the larger and more complex policies.

\mohawk is very efficient in finding errors in all the three test
suites, although each of them belong to a different complexity
class. This further underlines the effectiveness of the
abstraction-refinement based technique in \mohawk. Also, having a
single technique that can perform well on large real-world policies
that belong to different complexity classes is also useful from the
point of view maintainability and extensibility of the tool.

\mohawk, although slower compared to MC and BMC for small size
policies, can be reliably used to analyze policies of very large
sizes. Moreover, \mohawk's abstraction-refinement step can be
configured based on the policy size and complexity. We ran \mohawk
with less aggressive abstraction-refinement for the smaller policies
and got performance comparable to BMC. Furthermore, since our
technique is not tied to specific model-checking algorithms, it can
used in conjunction with other algorithms such as RBAC-PAT's forward
reachability.

\subsubsection{\bf Results on Simple Policies}

We first analyzed three ARBAC policies that were used in prior
work~\cite{scott07,rbacpat}, and the results are summarized in
Table~\ref{tab:simple}. The first and second policies did not satisfy
separate administration restriction, so we removed \canAssign
roles that have the administrative roles as target and used the
modified policies in our evaluation.

BMC, RBAC-PAT, and \mohawk were effective for all the
three policies. The absolute differences in time taken to verify are
not very significant because they are less than a second.

\mohawk with aggressive abstraction-refinement (Note that the degree
of abstraction-refinement can be configured by the user) is faster
compared to RBAC-PAT's forward reachability, but slower compared to
BMC and RBAC-PAT's backward reachability.  However, the absolute slow
down in each case is less than a second and is imperceptible to the
user. The reason for the slowdown experienced by \mohawk with
aggressive abstraction-refinement for these policies is that these
policies are so small that BMC can analyze them easily, while \mohawk
takes multiple iterations to arrive at the same answer. In other
words, the policies are too simple, and the abstraction-refinement
step creates unnecessary overhead. For the third test case, MC timed
out. Both RBAC-PAT and \mohawk with aggressive abstraction-refinement
are slower compared to BMC, and \mohawk is faster compared to
RBAC-PAT's forward reachability algorithm and slightly slower compared
to RBAC-PAT's backward reachability.

\sloppypar{ 

  We also ran \mohawk with different configuration of
  abstraction-refinement on these policies. It turns out that the less
  aggressive the abstraction-refinement step, the faster \mohawk gets
  for these small policies. In the limit it has similar performance as
  BMC.  }

